Probability-Flow ODE in Infinite-Dimensional Function Spaces

Recent advances in infinite-dimensional diffusion models have demonstrated their effectiveness and scalability in function generation tasks where the underlying structure is inherently infinite-dimensional. To accelerate inference in such models, we derive, for the first time, an analog of the probability-flow ODE (PF-ODE) in infinite-dimensional function spaces. Leveraging this newly formulated PF-ODE, we reduce the number of function evaluations while maintaining sample quality in function generation tasks, including applications to PDEs.

==> section/A04.tex <==


\section{Additional experiments}



\paragraph{2D Darcy flow} We consider a Darcy type equation of the form 
\begin{align*}
   \left\{ 
   \begin{aligned}
        -\nabla \cdot ( a \nabla u) = &f \quad \text{ on } \mathcal{O}= [0,1]^2, \\ 
        u =& 0 \quad \text{ on }\partial  \mathcal{O}. 
   \end{aligned}\right.
\end{align*}




\begin{figure}[H]
\centering
% 1행 3열
\begin{subfigure}{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/2D/Darcy/GTDarcy0.01.png}
    \caption{Ground Truth}
    \label{fig:Darcy-1(a)}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
    \centering
\includegraphics[width=\textwidth]{figures/2D/Darcy/samples64_ode_70bessel.png}
    \caption{ODE samples}
    \label{fig:Darcy-1(b)}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/2D/Darcy/samples64_sde_70bessel.png}
    \caption{SDE samples}
    \label{fig:Darcy-1(c)}
\end{subfigure}

\caption{Ground truth solution of Darcy type equation and synthetic solution from \{ODE, SDE\} methods. }
\label{fig:Darcy-1}
\end{figure}


Figure ~\ref{fig:Darcy-1(a)} shows ground truth solutions for the preceding Darcy type equation. Figure~\ref{fig:Darcy-1(b)} and Figure~\ref{fig:Darcy-1(c)} show synthetic solutions from ODE sampling and SDE sampling with the same checkpoint and same NFE=100, respectively. These samples are non-cherry-picked. We note here that samples via SDE solving are noisier than samples via ODE solving. From Figure~\ref{fig:Darcy-Qualitative}, one can observe that the sample qualities of ODE samples are better than sample qualities of SDE samples.

\begingroup
\allowdisplaybreaks
\begin{figure}[H]
\centering

% ODE
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/2D/Darcy/samples64_ode_5bessel.png}
%\caption{Caption 1}
%\label{fig:subfig1}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/2D/Darcy/samples64_ode_25bessel.png}
% \caption{Caption 2}
% \label{fig:subfig2}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/2D/Darcy/samples64_ode_50bessel.png}
%\caption{Caption 3}
% \label{fig:subfig3}
\end{subfigure}

\vspace{1em} 
% SDE 
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/2D/Darcy/samples64_sde_5bessel.png}
%\caption{Caption 4}
% \label{fig:subfig4}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/2D/Darcy/samples64_sde_25bessel.png}
%\caption{Caption 5}
% \label{fig:subfig5}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/2D/Darcy/samples64_sde_50bessel.png}
%\caption{Caption 6}
% \label{fig:subfig6}
\end{subfigure}

\caption{Qualitative comparison of ODE samples and SDE samples for Darcy type equation. (Top) Samples from ODE methods with NFEs=\{5, 25, 50\}. (Bottom) Samples from SDE methods with NFEs=\{5, 25, 50\}.} 
\label{fig:Darcy-Qualitative}
\end{figure}
\endgroup




\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/3D/heat/real64_ode_100bessel3d.png}
    \caption{Time evolution of ground truth solutions of diffusion-reaction equation.}
    \label{fig:heat3d}
\end{figure}



\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/3D/heat/samples64_ode_10bessel3d.png}
    \caption{ODE samples NFE = 10}
    \label{fig:heat3dODE10}
\end{figure}




\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/3D/heat/samples64_sde_10bessel3d.png}
    \caption{SDE samples NFE = 10}
    \label{fig:heat3dSDE10}
\end{figure}












\iffalse
\paragraph{3D diffusion-reaction} \textcolor{red}{This may be moved to appendix. Also some of the experiments may be modified and improved.} By conidering a solution of diffusion-reaction equation on two-dimensional spacial domain as a three-dimensional function, we can sample a time-evolving solution of diffusion-reaction equation (cf. Figure~\ref{fig:3dReacdiff}). Figure ~\ref{fig:3dReacdiff-ODE} shows time-evolving synthetic solutions of diffusion-reaction equations generated via solving the PF-ODE in the function space. 


\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{figures/2D/reacdiff_GT.png}
    \caption{Time evolution of ground truth solutions of diffusion-reaction equation.}
    \label{fig:3dReacdiff}
\end{figure}



\begin{figure}[H]
    \centering    \includegraphics[width=\linewidth]{figures/2D/samples64ODEbessel3d.png}
    \caption{Synthetic samples obtained from ODE solving with NFE = 200.}
    \label{fig:3dReacdiff-ODE}
\end{figure}

\fi


==> section/A__trash.tex <==
\section{Demystifying infinite dimensional SDEs} 
\label{app:demystify-sde}
In this section, explain that infinite-dimensional modeling can enhance the scalability of diffusion models, as an infinite-dimensional SDE can be viewed as a system of infinitely many finite-dimensional SDEs. 



Let $\{(\phi_n, \lambda_n)\}_{n \in \NN}$ be an eigensystem of $Q$ (which is a self-adjoint, positive operator). Consider a system of (one-dimensional) stochastic differential equations 
\begin{align*}
    dX_t^n = b_n(t) X_t^n dt + \lambda_n^{1/2} \sigma_n(t) dB_t^n, \quad t \in [0, T], n \in \NN, 
\end{align*}
where $b_n: [0, T] \to\RR$ and $\sigma_n: [0, T] \to \RR_{\ge 0}$. Here, $\{B^n = (B_t^n)_{t \ge 0}\}_{n \in \NN}$ is a collection of independent real-valued standard Brownian motion. Let us consider an $\mathcal{H}$-valued process 
\begin{align*}
    X_t  = \sum_{n = 1}^\infty X_t^n \phi_n, \quad t \in [0, T]. 
\end{align*}
Let 
\begin{align*}
    B(t, X_t) = \sum_{n = 1}^\infty b_n(t) \langle X_t, \phi_n\rangle_{\mathcal{H}} \phi_n = \sum_{n = 1}^\infty b_n(t) X_t^n \phi_n,
\end{align*}
and let $G(s)\phi_n = \sigma_n(s) \phi_n$ for all $n \ge 1$. By linearly extending the preceding equality, one has a mapping $G(\cdot) : [0, T] \to \mathscr{L}(\mathcal{H})$. Under this setting, it is easy to check that 
\begin{align*}
    dX_t = B(t, X_t) dt+ G(t) dW_t, \quad t \in [0, T]. 
\end{align*}
To see why, it suffices to note that 
\begin{align*}
    X_t &= \sum_{n = 1}^\infty X_t^n \phi_n = \sum_{n = 1}^\infty \left(
    X_0^n + \int_0^t b(s) X_s^n ds + \int_0^t \lambda_n^{1/2} \sigma_n(s) dB_s^n 
    \right) \phi_n \\
    &= \sum_{n = 1}^\infty X_0^n \phi_n + \int_0^t \sum_{n =  1}^\infty b(s)  X_s^n\phi_n \, ds + \sum_{n = 1}^\infty \left( \int_0^t \lambda_n^{1/2} \sigma_n(s) dB_s^n \right)\phi_n \\
    &= X_0 + \int_0^t B(s, X_s) \, ds + \sum_{n = 1}^\infty \int_0^t G(s) \phi_n \, d \langle W_s, \phi_n\rangle_{\mathcal{H}} \\
    &= X_0 + \int_0^t B(s, X_s) \, ds + \int_0^t G(s) \, dW_s. 
\end{align*}
Here, the last equality follows from Lemma 2.9 of \cite{gawarecki2011stochastic}. In particular, if $B(t, \cdot) = b(t) id_\mathcal{H}$ and $G(t) = \sigma(t) id_\mathcal{H}$, then the system of SDEs 
\begin{align}
    dX_t^n = b_n(t) X_t^n dt + \lambda_n^{1/2} \sigma_n(t) dB_t^n, \quad t \in [0, T], \  n \in \NN 
    \label{eq:system}
\end{align}
fully recovers the original SDE in $\mathcal{H}$. For example, the VP-SDE given by 
\begin{align*}
    dX_t = - \frac{\beta(t)}{2} X_t dt + \sqrt{\beta(t)}  dW_t, \quad X_0 \sim \PP_0, 
\end{align*}
and the sub-VP-SDE given by 
 \begin{align*}
        dX_t = -\frac{\beta(t)}{2} X_t \, dt + \sqrt{\beta(t) \left(1 - e^{-2\int_0^t \beta(s) ds} \right)} \, dW_t, \quad X_0 \sim \PP_0 
\end{align*}
can be viewed as a system of infinitely many stochastic equations in $\RR$. This type of analysis connects diffusion models in $\mathcal{H}$ with stochastic equations in the spectral domain \citep{phillips2022spectral}. 

When running an algorithm, one approximates the infinte-dimensional SDE of concern with the system of finite-dimensional SDEs 
\begin{align*}
    \bigg\{dX_t^n = b_n(t) X_t^n dt + \lambda_n^{1/2} \sigma_n(t) dB_t^n\bigg\}_{n = 1}^M, 
\end{align*}
with $M < \infty$. Because one can choose $M$ depending on available compute resource, infinite-dimensional SDE can enhance the scalability of the algorithm.   

The following proposition demystifies the logarithmic derivative $\rho_{\mathcal{H}_Q}^{\mu_t}$ in a specific setting. Althouth this result is not directly applied in an empirical study of this work, it may still serve a independent interst. 

\begin{proposition}
     Let $\mu_t$ be the law of $X_t = \sum_{n  =1}^\infty X_t^n \phi_n$ for $t \in (0, T]$. The logarithmic gradient $\rho_{\mathcal{H}_Q}^{\mu_t}$ of $\mu_t = \operatorname{Law}(X_t)$ in the Cameron-Martin space $\mathcal{H}_Q$ is given by 
    \begin{align*}
        \rho_{\mathcal{H}_Q}^{\mu_t}(u) = \sum_{n =1}^\infty \lambda_n^{} \partial_{\hat{u}(n)} \log p_t^{{(n)}} (\hat{u}(n)) \phi_n, \quad \forall u \in \mathcal{H}, 
    \end{align*}
where $p_t^{(n)}$ is the density of the pushforward of $\mu_t$ under the map $h \mapsto \langle h, \phi_n\rangle_{\mathcal{H}}$. 
    \label{prop:coordinate}
\end{proposition}



Let $p_t^{(n)}$ be the density of $X_t^n$ at pseudotime $t$. For the sake of notational simplicity, we denote by $\hat{u}(n)$ the $n$-th Fourier coefficient of $u \in \mathcal{H}$ with respect to the orthonormal basis $\{\phi_n\}_{n \in \NN}$, i.e., $\hat{u}(n) = \langle u, \phi_n\rangle_\mathcal{H}$. Before proving \propref{prop:coordinate}, we first state and prove an auxillary 

\begin{lemma}
    The logarithmic derivative $\rho_{\xi}^{\mu_t}$ of $\mu_t$ along the vector $\xi \in \mathcal{H}_Q$ is given by 
    \begin{align*}
        \rho_\xi^{\mu_t} (u) = \sum_{n = 1}^\infty \lambda_n^{1/2} \partial_{\hat{u}(n)} \log p_t^{(n)} (\hat{u}(n)) \langle Q^{-1/2}\xi, \phi_n\rangle_{\mathcal{H}}. 
    \end{align*}
    \label{lem:coordinate-aux}
\end{lemma}

\begin{proof}[Proof of \lemref{lem:coordinate-aux}] 
Let 
\begin{align*}
    \Tilde{\varrho}_\xi(u) = \sum_{n = 1}^\infty \lambda_n^{1/2} \partial_{\hat{u}(n)} \log p_t^{(n)} (\hat{u}(n)) \langle Q^{-1/2}\xi, \phi_n\rangle_{\mathcal{H}}. 
\end{align*}
One has to check that 
\begin{align*}
    \int_\mathcal{H} \left< D f_{\varphi_1, \cdots, \varphi_m} (u), \xi \right>_{\mathcal{H}_Q} \mu_t(du) = - \int_\mathcal{H} f_{\varphi_1, \cdots, \varphi_m}(u) \Tilde{\varrho}_\xi(u) \mu_t(du), 
\end{align*}
for all $f_{\varphi_1, \cdots, \varphi_m} \in \mathcal{FC}_b^\infty(\mathcal{H})$. It suffices to prove the preceding equality for $f_{\phi_1, \cdots, \phi_m}$ where $\{\phi_n\}_{n =1}^\infty$ is orthonormal basis of $\mathcal{H} $ consisting of eigenvectors of $Q$. Notice that
\begingroup
\allowdisplaybreaks
\begin{align*}
    &\int_\mathcal{H} \left< D f_{\phi_1, \cdots, \phi_m} (u), \xi \right>_{\mathcal{H}_Q} \mu_t(du) \\
    =& \int_\mathcal{H} \sum_{i = 1}^m (\partial_i f)(\phi_1(u), \cdots, \phi_m(u)) \langle \xi, Q\phi_i\rangle_{\mathcal{H}_Q} \, \mu_t(du) \\
    =& \sum_{i = 1}^m \int_\mathcal{H} (\partial_i f) (\hat{u}(1), \cdots, \hat{u}(m)) \langle \xi, Q\phi_i \rangle_{\mathcal{H}_Q} \, \mu_t(du) \\
    =& \sum_{i =1}^m \langle \xi, Q\phi_i \rangle_{\mathcal{H}_Q} \underbrace{\int_\RR \cdots \int_\RR}_{m\text{-times}} (\partial_i f)(x_1, \cdots, x_m) \left\{
    \prod_{i = 1}^m p_t^{(i)}(x_i) 
    \right\}\, dx_1 \cdots dx_m \\
    =& - \sum_{i= 1}^m \langle \xi, Q\phi_i \rangle_{\mathcal{H}_Q} \underbrace{\int_\RR \cdots \int_\RR}_{m\text{-times}} f(x_1, \cdots, x_m) \, \partial_{x_i} \left\{
    \prod_{i = 1}^m p_t^{(i)}(x_i) 
    \right\}\, dx_1 \cdots dx_m \\
    =& -\sum_{i = 1}^m \langle \xi, Q\phi_i\rangle_{\mathcal{H}_Q} \underbrace{\int_ \RR \cdots \int_\RR}_{m\text{-times}} f(x_1, \cdots, x_m) \left\{
    \prod_{i = 1}^m p_t^{(i)}(x_i) 
    \right\}\ \partial_{x_i} \log p_t^{(i)} (x_i) \, dx_1 \cdots dx_m.
\end{align*}
\endgroup
On the other hand, 
\begingroup
\allowdisplaybreaks
\begin{align*}
    &- \int_\mathcal{H} f_{\phi_1, \cdots, \phi_m}(u) \Tilde{\varrho}_\xi(u) \mu_t(du) \\
    =& - \int_\mathcal{H} f(\hat{u}(1), \cdots, \hat{u}(m)) \left[ 
    \sum_{n = 1}^\infty \lambda_n^{1/2} \, \partial_{\hat{u}(n)} \log p_t^{(n)} (\hat{u}(n)) \langle Q^{-1/2}\xi, \phi_n \rangle_\mathcal{H}
    \right] \mu_t(du)  \\
    =& -\sum_{n = 1}^\infty \lambda_n^{1/2} \langle Q^{-1/2} \xi, \phi_n\rangle_{\mathcal{H}} \int_\mathcal{H} f(\hat{u}(1), \cdots, \hat{u}(n)) \, \partial_{\hat{u}(n)} \log p_t^{(n)} (\hat{u}(n))  \, \mu_t(du) \\
    =& - \sum_{n = 1}^\infty \langle \xi, Q\phi_i\rangle_{\mathcal{H}_Q} \int_\mathcal{H} f(\hat{u}(1), \cdots, \hat{u}(n)) \, \partial_{\hat{u}(n)} \log p_t^{(n)} (\hat{u}(n))  \, \mu_t(du) \\
    =& -\sum_{i = 1}^m \langle \xi, \phi_i\rangle_{\mathcal{H}_Q} \underbrace{\int_ \RR \cdots \int_\RR}_{m\text{-times}} f(x_1, \cdots, x_m) \left\{
    \prod_{i = 1}^m p_t^{(i)}(x_i) 
    \right\}\ \partial_{x_i} \log p_t^{(i)} (x_i) \, dx_1 \cdots dx_m.
\end{align*}
\endgroup
Here, to clarify, 
\begin{align*}
    \lambda_n^{1/2} \langle Q^{-1/2} \xi, \phi_n\rangle_\mathcal{H} = \lambda_n \langle Q^{-1/2} \xi, Q^{-1/2} \phi_n\rangle_{\mathcal{H}}  = \lambda_n \langle \xi, \phi_n\rangle_{\mathcal{H}_Q} = \langle \xi, Q\phi_n\rangle_{\mathcal{H}_Q}. 
\end{align*}
Therefore, one concludes $\Tilde{\varrho}_\xi = \rho_\xi^{\mu_t}$, hence the claim. 
\end{proof}




\begin{proof}[Proof of \propref{prop:coordinate}]
In order to prove the proposition, it suffices to observe that for $\xi = Q^{1/2}\omega \in \mathcal{H}_Q$ ($\omega \in \mathcal{H}$), 
\begingroup
\allowdisplaybreaks
\begin{align*}
    \rho_\xi^{\mu_t}(u) &= \sum_{n = 1}^\infty \lambda_n^{1/2} \partial_{\hat{u}(n)} \log p_t^{(n)} (\hat{u}(n)) \langle Q^{-1/2}\xi, \phi_n\rangle_{\mathcal{H}} \\
    &= \sum_{n = 1}^\infty \lambda_n^{1/2} \partial_{\hat{u}(n)} \log p_t^{(n)} (\hat{u}(n)) \langle \omega, \phi_n\rangle_\mathcal{H} \\
    &= \sum_{n = 1}^\infty \frac{1}{\lambda_n} \left( 
    \partial_{\hat{u}(n)} \log p_t^{(n)} (\hat{u}(n)) \lambda_n \phi_n 
    \right) \lambda_n^{1/2} \langle \omega, \phi_n \rangle_\mathcal{H} \\
    &= \left<
    Q^{-1/2} \left( 
    \sum_{n = 1}^\infty \partial_{\hat{u}(n)} \log p_t^{(n)} (\hat{u}(n)) \lambda_n \phi_n
    \right), \ Q^{-1/2} \left(\sum_{k = 1}^\infty \lambda_k^{1/2} \langle \omega, \phi_k \rangle \phi_k \right)
    \right>_\mathcal{H} \\
    &= \Bigg<
     \sum_{n = 1}^\infty \partial_{\hat{u}(n)} \log p_t^{(n)} (\hat{u}(n)) \lambda_n \phi_n, \ \underbrace{\sum_{k = 1}^\infty \lambda_k^{1/2} \langle \omega, \phi_k \rangle \phi_k}_{= \xi}
    \Bigg>_{\mathcal{H}_Q}, 
\end{align*}
\endgroup
which directly proves the claim. 
\end{proof}

\iffalse

\vspace{5mm}

\subsection{Proof of \lemref{lemma:continuous}}
\label{app:proof-lem-continuous}
In this subsection, we rigorously state \lemref{lemma:continuous} and provide its proof. We first state the formal version of \lemref{lemma:continuous} as 

\begin{lemma}[Formal version of \lemref{lemma:continuous}] Consider an ODE in $\mathcal{H}$ with random initial point given by 
\begin{align*}
    dY_t = \mathcal{G}(t, Y_t) dt , \quad Y_0 \sim \PP_0, 
\end{align*}
where $\mathcal{G}(t, \cdot) : \mathcal{H} \to \mathcal{H}$ is continuous for any $t \in [0, T]$. 
If $\operatorname{supp}(\PP_0) \subset \mathcal{K}$ for some closed linear space $\mathcal{K} \subset \mathcal{H}$, $\operatorname{Ran}(\mathcal{G}_t|_\mathcal{K}) \subset \mathcal{K}$, and if every $f \in \mathcal{K}$ is continuous, then 
$\mathcal{A}^{0 \to t} f $ for all $f \in \mathcal{H}$ sampled from $\PP_0.$ Here, $\mathcal{A}^{0 \to t}f$ is the flow operator defined as in \eqref{eqn:flow}. 
\end{lemma}

\kunwoo{Maybe it will be better to state when $\mathcal{G}$ is continuous in space. Also maybe we have to modify the statement.} 


\begin{proof} 
First, we note that for any $s \in (0, t)$ one has that $f + s \mathcal{G}(0, f)$ lies in $\mathcal{K}$, provided that $f \in \gK$. By an inductive argument, for any partition $\tau  = (t_1, \cdots, t_\ell)$ of $[0,t]$ (where $t_i < t_{i + t}$ for all $i = 1, 2, \cdots, \ell - 1$ and $t_1 = 0, t_\ell = t$), one observes that
\begin{align*}
    \mathcal{A}_{\tau}^{0 \to t} f = f + \sum_{\ell = 1}^{n - 1} \Delta t_\ell \,  \mathcal{G}\left(t_{\ell}, \mathcal{A}_{(t_1, \cdots, t_{\ell})}^{0 \to t_\ell}f \right)
\end{align*}
lies in $\mathcal{K}$, where $\Delta t_\ell = t_{\ell + 1} - t_{\ell}$. 
Now, let $\{\tau_n\}_{n = 1}^\infty$ be a sequence of partitions of $[0, t]$, where $\tau_n = (t^n_{\ell_1}, \cdots, t^n_{\ell_n})$, and 
\begin{align*}
    |\tau_n| = \max \left\{\Delta t_{\ell} : \ell = 1,2, \cdots, n - 1 
 \right\}\xrightarrow[n \nearrow \infty]{} 0.  
\end{align*}
It is clear from the definition of Bochner integral that 
\begin{align*}
    \mathcal{A}_{\tau_n}^{0 \to t} f \xrightarrow[n \nearrow \infty]{} \mathcal{A}^{0 \to t} f 
\end{align*}
in $\mathcal{H}$. As $\mathcal{A}_{\tau_n}^{0 \to t} f \in \mathcal{K}$ for all $n = 1,2 , \cdots$, it follows that $\mathcal{A}^{0 \to t}f \in \mathcal{K}$. As our choice of $t \in (0, T]$ was arbitrary, the proof is now complete. 

\end{proof}

\fi 






%%%%%%%%%%%%%%


\subsection{Stochastic (Bochner) Integrals}


\kunwoo{I will rewrite this section completely} 

\paragraph{Bochner Integral and Martingales} Let $(X, \norm{\cdot})$ be a Banach space over $\Bbbk = \RR$ or $\Bbbk = \CC$. Denote by ${X}^\ast$ the dual space of ${X}$. Let $I \subset [0, \infty)$ be an interval, and let $\mathcal{M}(I)$ be the Lebesgue-measurable sets in $I$. The theory of Bochner integrals is concerned with the integration of vector-valued functions $f : I \to X$, i.e., functions whose values lie in the Banach space (which is possibly infinite-dimensional). 

\begin{definition}
    A function $f : I \to X$ is called \textbf{simple} if it can be written in the form 
    \begin{align*}
        f = \sum_{k = 1}^n x_k \mathds{1}_{A_k}, 
    \end{align*}
    where $x_k  \in X$ and $A_k \in \mathcal{M}(I)$ for each $k = 1,2, \cdots, n$.  
\end{definition}

As in the ordinary Lebesgue integrals, one defines the integral of simple function by 
\begin{align*}
    \int_I  \sum_{k = 1}^n x_k \mathds{1}_{A_k}(s) \, d m(s) = \sum_{k= 1}^n x_k m(A_k). 
\end{align*}


\begin{definition}
    A function $f : I \to X$ is called Bochner integrable if there exists a sequence $(f_n)_{n \in \NN}$ of simple functions such that $f_n(s) \to f(s)$ as $n \to \infty$ for Lebesgue-almost every $s \in I$ and such that 
    \begin{align*}
        \int_I \norm{f(s) - f_n(s)} \, m(ds) \to 0
    \end{align*}
    as $n \to \infty$. For Bochner integrable function $f$, one defines 
    \begin{align*}
        \int_I f(s) \, d m (s) = \lim_{n \to \infty} \int_I f_n (s) m(ds)
    \end{align*}
\end{definition}
\textit{Remark.} It could be proved that $\int_I f(s) \, d m(s) $ is independent of the choice of the sequence of simple functions $(f_n)_{n \in \NN}$.




\begin{definition}
    Let $M = (M_t)_{t\ge 0}$ be a stochastic process on $(\Omega, \mathcal{F}, \PP)$ with values in a separable Banach space $X$, and let $(\mathcal{F}_t)_{t \ge 0}$ be a filtration on $(\Omega, \mathcal{F}, \PP)$. The process $M$ is called an $(\mathcal{F}_t)_{t \ge 0}$-martingale, if 
    \begin{itemize}
        \item[1.] $\mathbb{E}[\|M_t\|] < \infty$ for all $t > 0$, 
        \item[2.] $M$ is adapted to $(\mathcal{F}_t)_{t \ge 0}$, 
        \item[3.] $\mathbb{E}[M_t \mid \mathcal{F}_s] = M_s$ $\mathbb{P}$-a.s. for all $0 \le s \le t < \infty$.  
    \end{itemize}
\end{definition}


The following theorem is a direct consequence of Doob's maximal inequality (which is a standard result in classical probability theory). 

\begin{theorem}[Maximal inequality] 
    Let $p \in (1, \infty)$ and let $X$ be a separable Banach space. If $M = (M_t)_{t \in [0, T]}$ is a right-continuous $X$-valued $(\mathcal{F}_t)$-martingale, then 
    \begin{align*}
        \mathbb{E}\left[ 
        \sup_{t \in [0, T]} \norm{M_t}^p
        \right]^{1/p } \le \frac{p}{p -1} \sup_{t \in [0, T]} \mathbb{E}\left[ \norm{M_t}^p\right]^{1/p} = \frac{p}{p - 1} \mathbb{E}[\norm{M_T}^p]^{1/p}. 
    \end{align*}
\end{theorem}
One usually takes $p = 2$. 



For $0 < T< \infty$, denote by $\mathcal{M}_T^2(X)$ the space of all $E$-valued continuous martingales that are square-integrable. Then, $\mathcal{M}_T^2(X)$ is equipped with the norm 
\begin{align*}
    \norm{M}_{\mathcal{M}_T^2(X)} := \sup_{t \in [0, T]} \mathbb{E}[\norm{M_t}_{X}^2]^{1/2}. 
\end{align*}
Furthermore, within this norm, $\mathcal{M}_T^2(E)$ is a Banach space.\footnote{Furthermore, if some regularity conditions on $E$ is added, then $\mathcal{M}_T^2(E)$ turns out to be a Hilbert space.}     

\paragraph{Construction of the Stochastic (Bochner) Integrals} 

We now provide an overview of the construction of the stochastic Bochner integrals. \\[3mm]

{\underline{\textbf{Step 1.}}} Define the class $\mathcal{E}$ of elemntary processes. 
\begin{definition}
    An $L = \mathscr{L}(\gU; \gH)$-valued process $\Phi_t$, $t \in [0, T]$, on a probability space $(\Omega, \mathcal{F}, \PP)$ equipped with a normal filtration $\mathcal{F}_t$, is called an \textbf{elementary process} if $\Phi$ is of the form 
    \begin{align*}
        \Phi_t (\omega) = \sum_{m = 0}^{k - 1} \Phi_m (\omega) \mathds{1}_{(t_m, t_{m + 1]}}(t), \quad \omega \in \Omega, t\in [0, T], 
    \end{align*}
    where $\Phi_m : \Omega \to L$ is $\mathcal{F}_{t_m}$-measurable with respect to the strong Borel $\sigma$-algebra on $L(\gU, \gH)$ for $0 \le m \le k - 1$, and $\Phi_m$ takes only a finite number of values in $L$ for $1 \le m \le k - 1$. 
\end{definition}
    It is clear that $\mathcal{E}$ is an $\RR$-vector space.\\[3pt]

    \underline{\textbf{Step 2.}} Define a ``linear isometry'' $\mathcal{E} \to \mathcal{M}_T^2$. To do so, we first have to define a norm on $\mathcal{E}$. \\[3pt]

    \underline{Define} the linear map $I: \mathcal{E} \to \mathcal{M}_T^2(E)$ by 
    \begin{align*}
        I[\Phi](t, \omega) := \int_0^t \Phi_s \, d W_s := \sum_{m = 0}^{k - 1} \Phi_m(W_{t_{m + 1} \wedge t} (\omega) - W_{t_m \wedge t}(\omega)). 
    \end{align*}
    Then, one can easily check that $I$ is well-defined, i.e., that $I$ is independent of the representation of $\Phi$. We will call $I$ a ``stochastic integral''. Of course, we wish to extend the notion of stochastic integral to more general class of processes. One can show that, the stochastic integral $\int_0^t \Phi_s \, dW_s $ is a continuous square-integrable martingale for $\Phi \in \mathcal{E}$. 


    \begin{definition} Let $\{e_k\}_{k \in \NN}$ be an orthonormal basis of $\gU$. An operator $A \in \mathscr{L}(\gU, \gH)$ is called a \textbf{Hilbert-Schmidt operator}, if 
    \begin{align*}
        \sum_{k\in \NN} \langle Ae_k, Ae_k \rangle_{\gH} < \infty. 
    \end{align*}
    \end{definition}
    Now, we consider the space $L_2 = \mathscr{L}_2(\gU, \gH)$ of all Hilbert-Schmidt operators $\gU \to \gH$. Then, $L_2$ is equipped with the inner product
    \begin{align*}
        \langle A, B \rangle_{L_2}  = \sum_{k \in \NN} \langle Ae_k, Be_k \rangle_{\gH}, \quad \forall A, B \in L_2. 
    \end{align*}
    Furthermore, $L_2$ is separable Hilbert space. 

    \begin{theorem}[An It\^o-isometry] 
        If $\Phi $ is an elementary $\mathscr{L}(\gU, \gH)$-valued process of the form 
        \begin{align*}
             \Phi_t (\omega) = \sum_{m = 0}^{k - 1} \Phi_m (\omega) \mathds{1}_{(t_m, t_{m + 1]}}(t), \quad \omega \in \Omega, t\in [0, T],
        \end{align*}
        then one has 
        \begin{align*}
            \norm{\int_0^\ast 
            \Phi_s \, dW_s 
            }_{\mathcal{M}_T^2}^2 = \mathbb{E}\left[ \int_0^T
            \norm{\Phi_s \circ Q^{1/2}}_{\mathscr{L}_2(\gU, \gH)}^2 ds 
            \right] =: \norm{\Phi}_{\mathcal{E}}^2. 
        \end{align*}
    \end{theorem}
Therefore, $I: \mathcal{E} \to \mathcal{M}^2_T(L)$ defines some sort of ``isometry.'' The functional $\mathcal{E} \ni \Phi \mapsto \norm{\Phi}_{\mathcal{E}} \in \RR$ is a norm (as the notation suggests). 


The proof of the preceding It\^o-isometry theorem could be done via a direct computation: by letting $\Delta_m= W_{t_{m+ 1}} - W_{t_m}$, one first expands  
    \begin{align*}
        \norm{\int_0^\ast \Phi_s \, dW_s}_{\mathcal{M}_T^2}^2 :&= \sup_{t \in [0, T]} \mathbb{E}\left[\norm{\int_0^t \Phi_s dW_s}_{\gH}^2 \right] = \mathbb{E} \left[
        \norm{\int_0^T \Phi_s \, dW_s}_{\gH}^2
        \right] \\
        &= \mathbb{E}\left[ 
        \norm{\sum_{m = 0}^{k - 1} \Phi_m \Delta_m}_{\gH}^2   
        \right] \\
        &= \sum_{m = 0}^{k - 1}\mathbb{E}\left[\norm{\Phi_m \Delta_m}_\gH^2\right] + 2\sum_{0 \le m < n \le k -1} \mathbb{E}\left[
        \left< \Phi_m \Delta_m, \Phi_n \Delta_n\right>_\gH
        \right]. 
    \end{align*}
    Then, one computes the second term of the very last equality by using monotone convergence theorem and Parseval's identity. 

    Now, recall that we wish to extend the definition of the stochastic integral $I : (\mathcal{E}, \norm{\cdot}_{\mathcal{E}}) \to (\mathcal{M}_T^2(L), \norm{\cdot}_{\mathcal{M}^2_T(L)})$. One way to do so is to take the closure $\overline{\mathcal{E}}$ of $\mathcal{E}$ (with respect to the norm $\norm{\cdot}_{\mathcal{E}}$) and then linearly extend $I$ onto $\overline{\mathcal{E}}$. To take the abstract closure, we have to give an explicit representation of $\overline{\mathcal{E}}$.\\[3pt]

     \underline{\textbf{Step 3.}} Give an explicit representation of $\overline{\mathcal{E}}$. \\[3pt]
Let $\gU_0 := Q^{1/2}(\gU)$ be the Cameron-Martin space of $\gU$ with respect to $\mathcal{N}(0, Q)$. We already know that $\gU_0$ is equipped with the inner product
\begin{align*}
    \langle u_0, v_0 \rangle_{0}:= \langle Q^{-1/2} u_0, Q^{-1/2} v_0 \rangle_{\gU}. 
\end{align*}
Also, we have a simple isometry: 
\begin{align*}
    \norm{T}_{\mathscr{L}_2(\gU_0, \gH)} = \norm{T \circ Q^{1/2}}_{\mathscr{L}_2(\gU, \gH)}. 
\end{align*}
For the sake of notational simplicity, denote by $L^0_2 $ the Hilbert space $\mathscr{L}_2(\gU_0, \gH)$.
 Additionally, define $\mathscr{L}(\gU,\gH)_0$ as
    \begin{align*}
        \mathscr{L}(\gU,\gH)_0 := \left\{ 
        T|_{\gU_0} \mathrel{\Big| } T \in \mathscr{L}(\gU, \gH) 
        \right\}. 
    \end{align*}
As $Q^{1/2} \in \mathscr{L}_2(\gU)$ (we already know this from the general theory), one has that $\mathscr{L}(\gU, \gH)_0 \subset L_2^0 = \mathscr{L}(\gU_0, \gH)$. Now, recall from \textbf{Step 2} that
\begin{align*}
     \norm{\int_0^\ast 
            \Phi_s \, dW_s 
            }_{\mathcal{M}_T^2}^2 = \mathbb{E}\left[ \int_0^T
            \norm{\Phi_s \circ Q^{1/2}}_{\mathscr{L}_2(\gU, \gH)}^2 ds 
            \right] = \norm{\Phi}_{\mathcal{E}}^2.
\end{align*}
Then, one can rewrite $\norm{\Phi}_{\mathcal{E}}$ as 
\begin{align*}
    \norm{\Phi}_{\mathcal{E}} =\mathbb{E}\left[ \int_0^T
            \norm{\Phi_s \circ Q^{1/2}}_{\mathscr{L}_2(\gU, \gH)}^2 ds 
            \right]^{1/2} = \mathbb{E}\left[
            \int_0^T \norm{\Phi_s}_{L_2^0}^2 ds 
            \right]^{1/2}. 
\end{align*}    


\underline{Define} $\mathcal{P}_T$ as 
    \begin{align*}
        &\mathcal{P}_T \\
        =& \sigma\left(\left\{
        (s, t] \times F_s \mathrel{\bigg|}0 \le s < t \le T, F_s \in \mathcal{F}_s
        \right\}
        \cup \left\{ \{0\} \times F_0 \mathrel{\bigg|} F_0 \in \mathcal{F}_0 \right\} 
        \right) \\
        =& \sigma\left(Y : \underbrace{\Omega_T}_{:= [0,T] \times \Omega} \to \RR \mathrel{\Bigg|} Y \text{ is left-continuous and adapted to } \mathcal{F}_t, t \in [0, T] \right). 
    \end{align*}
\begin{proposition}
    One has that
    \begin{align*}
        \overline{\mathcal{E}} &= \left\{
        \Phi :\Omega_T \to L_2^0 \mathrel{\bigg|} \Phi \text{ is predictable and } \norm{\Phi}_{\mathcal{E}} < \infty  
        \right\}\\ 
        &= L^2([0, T] \times \Omega, \mathcal{P}_T, dt \otimes \mathbb{P}; L_2^0)=: \mathcal{N}_W^2(0, T; \gH). 
    \end{align*}
\end{proposition}


 \underline{\textbf{Step 4.}} Extend the stochastic integral to the linear space $\mathcal{N}_W(0, T; \gH)$. \\[3pt]

    This could be done via a so-called ``localization technique.''. One can extend the definition of the stochastic integral to the linear space
    \begin{align*}
        &\mathcal{N}_W(0, T; \gH)\\
        := &\left\{ 
        \Phi : \Omega_T \to L_2^0 \mathrel{\Bigg|} \Phi \text{ is predictable and } \mathbb{P}\left( 
        \int_0^T \norm{\Phi_s}_{L^0_2}^2 ds  < \infty 
        \right) = 1
        \right\}. 
    \end{align*}
    Elements of the space $\mathcal{N}_W(0, T; \gH)$ is called \textbf{stochastically integrable}. The extension could be done in the following fashion: For any $\Phi \in \mathcal{N}_W(0, T; \gH)$, define 
    \begin{align*}
        \tau_n := \inf\left\{ 
        t  \in [0, T] \mathrel{\Bigg|} \int_0^t \norm{\Phi_s}_{L^0_2}^2 ds > n
        \right\} \wedge T. 
    \end{align*}
    One can observe that $(\tau_n)_{n \in \NN}$ is an increasing sequence of stopping times. Then, for $\Phi \in \mathcal{N}_W(0, T; \gH)$, one can define the stochastic integrals for $t \in [0, T]$: 
        \begin{align*}
            (t, \omega) \mapsto \left(\int_0^t \mathds{1}_{(0, \tau_n]}(s) \Phi_s dW_s\right)(\omega), \quad n \in \NN. 
        \end{align*}
        Then, for an arbitrary $t \in [0, T]$, set 
        \begin{align*}
            \int_0^t \Phi_s dW_s := \int_0^t \mathds{1}_{(0, \tau_n]}(s) \Phi_s dW_s 
        \end{align*}
        for any $n \in \NN$ such that $\tau_n \ge t$. Then, this definition is consistent. 
        

\vspace{8mm}









\iffalse
\begin{wrapfigure}{r}{0.47\textwidth}
  \begin{center}    \includegraphics[width=0.7\linewidth]{figures/2D/reacdiff/sde_vs_ode_reacdiff.png}
  \end{center}
    \caption{SW distance vs. NFE}
    \label{fig:reacdiff2D-quantitative}
\end{wrapfigure}
\fi



